Modeling Ambient Scene Dynamics for Free-view Synthesis

We introduce a novel method for dynamic free-view synthesis of an ambient scenes from a monocular capture bringing a immersive quality to the viewing experience. Our method builds upon the recent advancements in 3D Gaussian Splatting (3DGS) that can faithfully reconstruct complex static scenes. Previous attempts to extend 3DGS to represent dynamics have been confined to bounded scenes or require multi-camera captures, and often fail to generalize to unseen motions, limiting their practical application. Our approach overcomes these constraints by leveraging the periodicity of ambient motions to learn the motion trajectory model, coupled with careful regularization. We also propose important practical strategies to improve the visual quality of the baseline 3DGS static reconstructions and to improve memory efficiency critical for GPU-memory intensive learning. We demonstrate high-quality photorealistic novel view synthesis of several ambient natural scenes with intricate textures and fine structural elements.

==> 6_conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}

==> figures/limitation.tex <==
\begin{figure*}[H]
\centering



\mpage{0.08}{\includegraphics[width=\linewidth, trim=260 0 260 0, clip]{images/unsplash_blur/input/asal-mshk-y8gfRMNd3as-unsplash.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/asal-mshk-y8gfRMNd3as-unsplash/view_010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours//asal-mshk-y8gfRMNd3as-unsplash/view_030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours//asal-mshk-y8gfRMNd3as-unsplash/view_080.png}}\hfill
%%%
\mpage{0.08}{\includegraphics[width=\linewidth, trim=260 0 260 0, clip]{images/limitations/id_00002529_blur/id_00002529.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/limitations/id_00002529_blur/view_010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/limitations/id_00002529_blur/view_030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/limitations/id_00002529_blur/view_080.png}}\hfill
%%%
\mpage{0.08}{\includegraphics[width=\linewidth, trim=260 0 260 0, clip]{images/unsplash_blur/input/brandon-atchison-eexdeq3NleQ-unsplash.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/brandon-atchison-eexdeq3NleQ-unsplash/view_010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/brandon-atchison-eexdeq3NleQ-unsplash/view_030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/brandon-atchison-eexdeq3NleQ-unsplash/view_080.png}}\\




% \mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{}}}  \hfill
\mpage{0.08}{\small{Input}}\hfill
\mpage{0.22}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~360$^\circ$ generation~~}}}$}\hfill
\mpage{0.08}{\small{Input}}\hfill
\mpage{0.22}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~360$^\circ$ generation~~}}}$}\hfill
\mpage{0.08}{\small{Input}}\hfill
\mpage{0.22}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~360$^\circ$ generation~~}}}$}\\
\vspace{-3mm}
\captionof{figure}{
\textbf{Limitations.}
Our approach inherits limitations from existing methods for shape reconstruction (missing leg and unusual hand shape (left)) and back-view synthesis (misaligned dress length due to lack of geometry awareness (middle)).
% and tilted legs (2nd row).
% \changil{I'd use ``top'' and ``middle'' rows instead of first and second rows.}
% back view issues
% \changil{Do we? In the previous sentence, the second row is about imperfect shape estimation.} \badour{removed to avoid confusion}
% We present a failure case attributed to the back-view synthesis (middle).
% Since the back-view synthesis approach~\cite{albahar2021pose} lacks the awareness of the underlying geometry, it may misalign the length of skirts, dresses, and other garments. 
% This can be observed where the legs appear textured with the garment pattern (middle).
% The back-view synthesis approach~\shortcite{albahar2021pose} lacks awareness of the underlying geometry, hence it may misalig the lengths of skirts, dresses, and other garments, as seen in the textured legs (middle).
We also show the baked specularity on the face texture, which is ideally view-dependent (right). 
% Our limitation
% We employ a progressive view synthesis approach, and our number of views $(N=8)$ is limited and does not guarantee coverage of all possible 360-degree regions.
% % \changil{Is it a limitation? This can be avoided simply by synthesizing more views?}
% As a result, certain regions may still be occluded and lack supervision, leading to random values being assigned, as seen in the area behind the arm in the bottom row.
% \changil{I cannot spot the mentioned artifact. Maybe we remove the third row?}\badour{picked a view that shows this better}
%
% Images from Unsplash.
}
\label{fig:limitation}
\end{figure*}

==> figures/limitation_v.tex <==
\begin{figure}[t]
\centering



\mpage{0.25}{\includegraphics[width=\linewidth, trim=260 0 260 0, clip]{images/unsplash_blur/input/asal-mshk-y8gfRMNd3as-unsplash.png}}\hfill
\mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/asal-mshk-y8gfRMNd3as-unsplash/view_010.png}}\hfill
\mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours//asal-mshk-y8gfRMNd3as-unsplash/view_030.png}}\hfill
\mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours//asal-mshk-y8gfRMNd3as-unsplash/view_060.png}}\hfill
\mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours//asal-mshk-y8gfRMNd3as-unsplash/view_080.png}}\\
%%
\vspace{1mm}
%%
\mpage{0.25}{\includegraphics[width=\linewidth, trim=260 0 260 0, clip]{images/limitations/id_00002529_blur/id_00002529.png}}\hfill
\mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/limitations/id_00002529_blur/view_010.png}}\hfill
\mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/limitations/id_00002529_blur/view_030.png}}\hfill
\mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/limitations/id_00002529_blur/view_060.png}}\hfill
\mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/limitations/id_00002529_blur/view_080.png}}\\
%%
% \mpage{0.25}{\includegraphics[width=\linewidth, trim=260 0 260 0, clip]{images/limitations/id_00005349/id_00005349.png}}\hfill
% \mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/limitations/id_00005349/view_008.png}}\hfill
% \mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/limitations/id_00005349/view_039.png}}\hfill
% \mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/limitations/id_00005349/view_050.png}}\hfill
% \mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/limitations/id_00005349/view_084.png}}\\

\vspace{1mm}
%%
\mpage{0.25}{\includegraphics[width=\linewidth, trim=260 0 260 0, clip]{images/unsplash_blur/input/brandon-atchison-eexdeq3NleQ-unsplash.png}}\hfill
\mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/brandon-atchison-eexdeq3NleQ-unsplash/view_010.png}}\hfill
\mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/brandon-atchison-eexdeq3NleQ-unsplash/view_030.png}}\hfill
\mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/brandon-atchison-eexdeq3NleQ-unsplash/view_060.png}}\hfill
\mpage{0.16}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/brandon-atchison-eexdeq3NleQ-unsplash/view_080.png}}\\




% \mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{}}}  \hfill
\mpage{0.25}{\small{Input}}\hfill
\mpage{0.73}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~360$^\circ$ generation~~}}}$}\\

\captionof{figure}{
\textbf{Limitations.}
As our approach builds upon off-the-shelf methods for human shape reconstruction and back-view synthesis, we inherit their limitations. 
% shape issues
Due to the imperfect shape estimation, our 360-degree generation in the top row exhibits a missing leg and an unusual hand shape (top row).
% and tilted legs (2nd row).
% \changil{I'd use ``top'' and ``middle'' rows instead of first and second rows.}
% back view issues
We present a failure case in the middle row attributed to the back-view synthesis. 
% \changil{Do we? In the previous sentence, the second row is about imperfect shape estimation.} \badour{removed to avoid confusion}
Since the back-view synthesis approach~\cite{albahar2021pose} lacks the awareness of the underlying geometry, it may misalign the length of skirts, dresses, and other garments. 
This can be observed where the legs appear textured with the garment pattern.
The bottom row shows the baked specularity on the face texture, which is ideally view-dependent. 
% Our limitation
% We employ a progressive view synthesis approach, and our number of views $(N=8)$ is limited and does not guarantee coverage of all possible 360-degree regions.
% % \changil{Is it a limitation? This can be avoided simply by synthesizing more views?}
% As a result, certain regions may still be occluded and lack supervision, leading to random values being assigned, as seen in the area behind the arm in the bottom row.
% \changil{I cannot spot the mentioned artifact. Maybe we remove the third row?}\badour{picked a view that shows this better}
%
Images from Unsplash.
}
\label{fig:limitation}
\end{figure}

==> figures/method_dynamic.tex <==
\begin{figure*}[t]    
\centering
\includegraphics[width=\linewidth]{images/dynamic-recon.png}
% \vspace{-4mm}
\caption{\textbf{Time-variant deformation.}
We utilize basis functions derived from the discrete cosine transform (DCT) to represent the time-variant deformation.
Given 3D center position of a Gaussian, we use a voxel-based encoder and MLP to predict the coefficient for each basis.
We take the linear combination of all these bases to obtain the final trajectory. 
The time-variant deformation $\Delta x_t$ and $\Delta q_t$ is sampled from the trajectory.
\chen{Just write a draft. Need some work.}
}
\label{fig:method-dynamic}
\end{figure*}


==> figures/nobackview.tex <==
\begin{figure}[t]
\centering

%%%% 
\mpage{0.10}{\includegraphics[width=\linewidth, trim=390 0 390 0, clip]{images/elicitdf_blur/input/id_00002818.png}}\hfill
\hspace{1mm}
\mpage{0.10}{\includegraphics[width=\linewidth, trim=390 0 390 0, clip]{images/elicitdf_blur/ours/id_00002818_nobackview/view_010.png}}\hfill
\mpage{0.10}{\includegraphics[width=\linewidth, trim=390 0 390 0, clip]{images/elicitdf_blur/ours/id_00002818_nobackview/view_030.png}}\hfill
\mpage{0.10}{\includegraphics[width=\linewidth, trim=390 0 390 0, clip]{images/elicitdf_blur/ours/id_00002818_nobackview/view_080.png}}\hfill
\hspace{2mm}
\mpage{0.10}{\includegraphics[width=\linewidth, trim=390 0 390 0, clip]{images/elicitdf_blur/ours/id_00002818/view_010.png}}\hfill
\mpage{0.10}{\includegraphics[width=\linewidth, trim=390 0 390 0, clip]{images/elicitdf_blur/ours/id_00002818/view_030.png}}\hfill
\mpage{0.10}{\includegraphics[width=\linewidth, trim=390 0 390 0, clip]{images/elicitdf_blur/ours/id_00002818/view_080.png}}\hfill
\\

\vspace{-2mm}
\mpage{0.06}{\small{Input}}\hfill
\mpage{0.4}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~Without back-view~~}}}$}\hfill
\mpage{0.4}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~Ours~~}}}$}\\
\vspace{-2mm}
\caption{\textbf{The need of back-view synthesis.}
% We validate our choice to initialize the back-view of the input image using an off-the-shelf human reposing technique.
Having an initial back-view encourages all other views to preserve the appearance of the person in the input image especially when a target view is far from the input view.
}
\label{fig:nobackview}
\end{figure}

==> figures/overview_multiviewsyn.tex <==
\begin{figure*}[t]    
\centering
\includegraphics[width=0.95\linewidth]{images/overview_multiviewsyn_blur.pdf}
\mpage{0.35}{{Initialization}}\hfill
\mpage{0.55}{{Shape-guided diffusion}}\\
\vspace{-1mm}
\caption{\textbf{Person image generation with shape-guided diffusion.}
% \changil{Is the diagram above about single-view synthesis, not the entire pipeline? The intro reads such that multiple inpainted views are blended into a coherent 3D model, which is not presented in the diagram above. Edit: Oh, I see the arrow from the ``output view'' to the ``support set'' now. But the pipeline in the diagram doesn't show the ``final output represetation'' or at least it's not clear what it is, if it's presented above.}
% Problem
To generate a 360-degree view of a person from a \emph{single} image $I_1$, we first synthesize multi-view images of the person. 
% initialization
We use an off-the-shelf method to infer the 3D geometry~\shortcite{saito2020pifuhd} and synthesize an initial back-view $\tilde{I}_N$ of the person~\shortcite{albahar2021pose} as a guidance.
% We initialize the back-view of the person to ensure that the synthesized views preserve the input appearance.
% set V
We add our input view $I_1$ and the synthesized initial back-view $\tilde{I}_N$ to our support set $V$.
% \jiabin{WHY do we generate back view first?}
% View consistency
To generate a new view $V_c$, we aggregate all the visible pixels from our support set $V$ 
% \changil{(we didn't mention those ``previously synthesized views'' but only the back view)} 
by blending their RGB color, weighted by visibility, viewing angles, and the distance to missing regions. 
%This ensures that the synthesized views are consistent with the existing views.
% Inpainting
To hallucinate the unseen appearance and synthesize view $\hat{I}_c$, we use a pretrained inpainting diffusion model guided by shape cues (normal $N_c$ and silhouette $S_c$ maps). 
% We add this generated view $\hat{I}_c$ to our support set and proceed to the next view until all the views are synthesized. 
We include the generated view $\hat{I}_c$ in our support set and repeat this process for all the remaining views.
% \jiabin{Can we visualize the support set?}
% guide the synthesis to respect the underlying 3D structure.
% % fusion
% Finally, we perform multi-view fusion by optimizing a UV texture map to obtain a 3D-consistent high-resolution human model (see our multi-view fusion in~\figref{multiviewfusion}).
}
\label{fig:multiviewsyn}
\end{figure*}


==> figures/results_df.tex <==
\begin{figure*}[t]
\centering

%%%% 
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/input/id_00001999.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00001999/010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00001999/030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00001999/080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00001999/pred_00000010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00001999/pred_00000030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00001999/pred_00000080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00001999/010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00001999/030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00001999/080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00001999/view_010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00001999/view_030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00001999/view_080.png}}\hfill
\\


%%%% 
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/input/id_00003079.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00003079/010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00003079/030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00003079/080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00003079/pred_00000010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00003079/pred_00000010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00003079/pred_00000010.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00003079/010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00003079/030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00003079/080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00003079/view_010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00003079/view_030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00003079/view_080.png}}\hfill
\\

%%%% 
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/input/id_00003980.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00003980/010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00003980/030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00003980/080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00003980/pred_00000010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00003980/pred_00000030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00003980/pred_00000080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00003980/010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00003980/030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00003980/080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00003980/view_010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00003980/view_030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00003980/view_080.png}}\hfill
\\


%%%% 
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/input/id_00005307.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00005307/010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00005307/030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00005307/080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00005307/pred_00000010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00005307/pred_00000030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00005307/pred_00000080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00005307/010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00005307/030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00005307/080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00005307/view_010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00005307/view_030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00005307/view_080.png}}\hfill
\\


%%%% 
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/input/id_00000089_17.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00000089_17/010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00000089_17/030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/pifu/id_00000089_17/080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00000089_17/pred_00000010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00000089_17/pred_00000030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/iper/id_00000089_17/pred_00000080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00000089_17/010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00000089_17/030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/texture/id_00000089_17/080.png}}\hfill
\hspace{2mm}
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00000089_17/view_010.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00000089_17/view_030.png}}\hfill
\mpage{0.065}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/df/ours/id_00000089_17/view_080.png}}\hfill
\\

\vspace{1mm}

\mpage{0.1}{\small{Input}}\hfill
\mpage{0.2}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~PIFu~\shortcite{saito2019pifu}~~}}}$}\hfill
\mpage{0.2}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~Impersonator++~\shortcite{liu2021liquid}~~}}}$}\hfill
\mpage{0.2}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~TEXTure~\shortcite{richardson2023texture}~~}}}$}\hfill
\mpage{0.2}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~Ours~~}}}$}\\

\caption{\textbf{Visual comparisons on the DeepFashion dataset (cont.).}
We compare our approach with prior methods~\cite{saito2019pifu,liu2021liquid,richardson2023texture} on the DeepFashion dataset~\cite{liuLQWTcvpr16DeepFashion}. 
Our results showcase photorealistic images with consistent views that are consistent with the input images.
We show the full 360-degree view generation results of more subjects in our \emph{supplementary material}.
% \changil{Add citations next to the baseline names above.}
% \changil{I see that we used the results of ELICIT that were provided by the authors in Figure 7, but why did we not use the same identities in Figure 6? It could be a single figure?}\badour{because in that subset are results are not great as in these results.}
% \changil{Do we have more results in the supplementary material? Let's mention it in the caption if we do.}
}
\label{fig:df}
\end{figure*}

==> figures/results_elicitdf.tex <==
\begin{figure}[t]
\centering
%0.045
% %%%% 
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/input/id_00007818.png}}\hfill
% \hspace{2mm}
% % \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/pifu/id_00007818/010.png}}\hfill
% % \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/pifu/id_00007818/030.png}}\hfill
% % \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/pifu/id_00007818/080.png}}\hfill
% % \hspace{2mm}
% % \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/iper/id_00007818/pred_00000010.png}}\hfill
% % \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/iper/id_00007818/pred_00000030.png}}\hfill
% % \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/iper/id_00007818/pred_00000080.png}}\hfill
% % \hspace{2mm}
% % \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/texture/id_00007818/010.png}}\hfill
% % \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/texture/id_00007818/030.png}}\hfill
% % \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/texture/id_00007818/080.png}}\hfill
% % \hspace{2mm}
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/elicit/id_00007818/000080.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/elicit/id_00007818/000060.png}}\hfill
% % \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/elicit/id_00007818/000030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/elicit/id_00007818/000010.png}}\hfill
% \hspace{2mm}
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/ours/id_00007818/view_010.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/ours/id_00007818/view_030.png}}\hfill
% % \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/ours/id_00007818/view_060.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/ours/id_00007818/view_080.png}}\hfill
% \\


%%%% 
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/input/id_00004235.png}}\hfill
\hspace{2mm}
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/pifu/id_00004235/010.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/pifu/id_00004235/030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/pifu/id_00004235/080.png}}\hfill
% \hspace{2mm}
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/iper/id_00004235/pred_00000010.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/iper/id_00004235/pred_00000030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/iper/id_00004235/pred_00000080.png}}\hfill
% \hspace{2mm}
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/texture/id_00004235/010.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/texture/id_00004235/030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/texture/id_00004235/080.png}}\hfill
% \hspace{2mm}
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/elicit/id_00004235/000080.png}}\hfill
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/elicit/id_00004235/000060.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/elicit/id_00004235/000030.png}}\hfill
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/elicit/id_00004235/000010.png}}\hfill
\hspace{2mm}
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/ours/id_00004235/view_010.png}}\hfill
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/ours/id_00004235/view_030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/ours/id_00004235/view_060.png}}\hfill
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/ours/id_00004235/view_080.png}}\hfill
\\

\vspace{-1mm}
%%%% 
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/input/id_00002818.png}}\hfill
\hspace{2mm}
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/pifu/id_00002818/010.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/pifu/id_00002818/030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/pifu/id_00002818/080.png}}\hfill
% \hspace{2mm}
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/iper/id_00002818/pred_00000010.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/iper/id_00002818/pred_00000030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/iper/id_00002818/pred_00000080.png}}\hfill
% \hspace{2mm}
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/texture/id_00002818/010.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/texture/id_00002818/030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/texture/id_00002818/080.png}}\hfill
% \hspace{2mm}
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/elicit/id_00002818/000080.png}}\hfill
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/elicit/id_00002818/000060.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/elicit/id_00002818/000030.png}}\hfill
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/elicit/id_00002818/000010.png}}\hfill
\hspace{2mm}
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/ours/id_00002818/view_010.png}}\hfill
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/ours/id_00002818/view_030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/ours/id_00002818/view_060.png}}\hfill
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/ours/id_00002818/view_080.png}}\hfill
\\
\vspace{-2mm}

%%%% 
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/input/id_00000000.png}}\hfill
\hspace{2mm}
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/pifu/id_00000000/010.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/pifu/id_00000000/030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/pifu/id_00000000/080.png}}\hfill
% \hspace{2mm}
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/iper/id_00000000/pred_00000010.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=400 0 300 0, clip]{images/elicitdf/iper/id_00000000/pred_00000030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/iper/id_00000000/pred_00000080.png}}\hfill
% \hspace{2mm}
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/texture/id_00000000/010.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/texture/id_00000000/030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/texture/id_00000000/080.png}}\hfill
% \hspace{2mm}
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/elicit/id_00000000/000080.png}}\hfill
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/elicit/id_00000000/000060.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf/elicit/id_00000000/000030.png}}\hfill
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/elicit/id_00000000/000010.png}}\hfill
\hspace{2mm}
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/ours/id_00000000/view_010.png}}\hfill
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/ours/id_00000000/view_030.png}}\hfill
% \mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/ours/id_00000000/view_060.png}}\hfill
\mpage{0.11}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/elicitdf_blur/ours/id_00000000/view_080.png}}\hfill
\\


\mpage{0.11}{\small{Input}}\hfill
\hspace{1mm}
% \mpage{0.117}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~PIFu~~}}}$}\hfill
% \hspace{1mm}
% \mpage{0.117}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~Impersonator++~~}}}$}\hfill
% \hspace{1mm}
% \mpage{0.117}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~TEXTure~~}}}$}\hfill
% \hspace{1mm}
\mpage{0.4}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~ELICIT \shortcite{huang2022one}~~}}}$}\hfill
\hspace{1mm}
\mpage{0.4}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~Ours~~}}}$}\\
\vspace{-3mm}

\caption{\textbf{Visual comparisons on the DeepFashion dataset.}
% We compare our 3D human digitization approach with ELICIT~\shortcite{huang2022one}, where its evaluation data and results were provided by the authors.
% It can be seen that our results are photorealistic, faithfully synthesizing novel views.
% See Figure~\ref{fig:df} for comparisons with other baselines and our \emph{supplementary material} for the full 360-degree results of more subjects.
We compare our approach to ELICIT~\shortcite{huang2022one}, using the authors' provided evaluation data and results. Our results achieve photorealism and faithfully synthesize novel views.
}
\label{fig:elicitdf}
\end{figure}

==> figures/results_thuman.tex <==
\begin{figure*}[t]
\centering


%%%% INPUT %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{Input}}}  \hfill
\mpage{0.061}{}\hfill
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/input/0014.png}}\hfill
\mpage{0.061}{}\hfill
\mpage{0.0725}{}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/input/0057.png}}\hfill
\mpage{0.0725}{}\hfill
\mpage{0.0725}{}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/input/0324.png}}\hfill
\mpage{0.0725}{}\hfill
\mpage{0.0675}{}\hfill
\mpage{0.055}{\includegraphics[width=\linewidth, trim=350 0 310 0, clip]{images/thuman_blur/input/0445.png}}\hfill
\mpage{0.0675}{}\hfill
\mpage{0.06}{}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/input/0088.png}}\hfill
\hspace{5mm}
\mpage{0.06}{}\\

\vspace{-1mm}

%%%% pws_baseline %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{PwS baseline}}}  \hfill
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/pws_baseline/0014/010.png}}\hfill
\hspace{-3mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/pws_baseline/0014/030.png}}\hfill
\hspace{-5mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/pws_baseline/0014/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pws_baseline/0057/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pws_baseline/0057/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pws_baseline/0057/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pws_baseline/0324/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pws_baseline/0324/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pws_baseline/0324/080.png}}\hfill
\hspace{2mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=300 0 300 0, clip]{images/thuman_blur/pws_baseline/0445/010.png}}\hfill
\hspace{-2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pws_baseline/0445/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pws_baseline/0445/080.png}}\hfill
\hspace{2mm}
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/pws_baseline/0088/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pws_baseline/0088/030.png}}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/pws_baseline/0088/080.png}}\\


\vspace{-1mm}


%%%% PIFu %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{PIFu}}}  \hfill
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/pifu/0014/010.png}}\hfill
\hspace{-3mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/pifu/0014/030.png}}\hfill
\hspace{-5mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0 0, clip]{images/thuman_blur/pifu/0014/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pifu/0057/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pifu/0057/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pifu/0057/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pifu/0324/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pifu/0324/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pifu/0324/080.png}}\hfill
\hspace{2mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=300 0 300 0, clip]{images/thuman_blur/pifu/0445/010.png}}\hfill
\hspace{-2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pifu/0445/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pifu/0445/080.png}}\hfill
\hspace{2mm}
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/pifu/0088/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/pifu/0088/030.png}}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/pifu/0088/080.png}}\\


\vspace{-0.6mm}


%%%% iper %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{Impersonator++}}}  \hfill
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/iper/0014/010.png}}\hfill
\hspace{-3mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/iper/0014/030.png}}\hfill
\hspace{-5mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/iper/0014/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/iper/0057/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/iper/0057/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/iper/0057/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/iper/0324/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/iper/0324/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/iper/0324/080.png}}\hfill
\hspace{2mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=300 0 300 0, clip]{images/thuman_blur/iper/0445/010.png}}\hfill
\hspace{-2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/iper/0445/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/iper/0445/080.png}}\hfill
\hspace{2mm}
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/iper/0088/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/iper/0088/030.png}}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/iper/0088/080.png}}\\


\vspace{-0.6mm}


%%%% texture %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{TEXTure}}}  \hfill
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/texture/0014/010.png}}\hfill
\hspace{-3mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/texture/0014/030.png}}\hfill
\hspace{-5mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/texture/0014/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/texture/0057/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/texture/0057/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/texture/0057/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/texture/0324/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/texture/0324/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/texture/0324/080.png}}\hfill
\hspace{2mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=300 0 300 0, clip]{images/thuman_blur/texture/0445/010.png}}\hfill
\hspace{-2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/texture/0445/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/texture/0445/080.png}}\hfill
\hspace{2mm}
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/texture/0088/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/texture/0088/030.png}}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/texture/0088/080.png}}\\


\vspace{-0.6mm}


%%%% Magic123 %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{Magic123}}}  \hfill
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/magic123/0014/010.png}}\hfill
\hspace{-3mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/magic123/0014/030.png}}\hfill
\hspace{-5mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/magic123/0014/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/magic123/0057/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/magic123/0057/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/magic123/0057/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/magic123/0324/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/magic123/0324/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/magic123/0324/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/magic123/0445/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/magic123/0445/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/magic123/0445/080.png}}\hfill
\hspace{2mm}
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/magic123/0088/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/magic123/0088/030.png}}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/magic123/0088/080.png}}\\

\vspace{-0.6mm}


%%%% S3F %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{S3F}}}  \hfill
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/s3f/0014/010.png}}\hfill
\hspace{-3mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/s3f/0014/030.png}}\hfill
\hspace{-5mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/s3f/0014/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/s3f/0057/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/s3f/0057/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/s3f/0057/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/s3f/0324/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/s3f/0324/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/s3f/0324/080.png}}\hfill
\hspace{2mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=300 0 300 0, clip]{images/thuman_blur/s3f/0445/010.png}}\hfill
\hspace{-2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/s3f/0445/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/s3f/0445/080.png}}\hfill
\hspace{2mm}
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/s3f/0088/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/s3f/0088/030.png}}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/s3f/0088/080.png}}\\


\vspace{-0.6mm}


%%%% ours %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{Ours}}}  \hfill
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/ours/0014/010.png}}\hfill
\hspace{-3mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/ours/0014/030.png}}\hfill
\hspace{-5mm}
\mpage{0.068}{\includegraphics[width=\linewidth, trim=250 0 290 0, clip]{images/thuman_blur/ours/0014/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/ours/0057/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/ours/0057/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/ours/0057/080.png}}\hfill
\hspace{2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/ours/0324/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/ours/0324/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/ours/0324/080.png}}\hfill
\hspace{2mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=300 0 300 0, clip]{images/thuman_blur/ours/0445/010.png}}\hfill
\hspace{-2mm}
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/ours/0445/030.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/ours/0445/080.png}}\hfill
\hspace{2mm}
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/ours/0088/010.png}}\hfill
\mpage{0.045}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/thuman_blur/ours/0088/030.png}}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=280 0 250 0, clip]{images/thuman_blur/ours/0088/080.png}}\\

\vspace{-2mm}


\caption{\textbf{Visual comparisons on the THuman2.0 dataset.}
We compare our approach with prior methods~\cite{saito2019pifu,liu2021liquid,richardson2023texture,albahar2021pose,corona2022structured,qian2023magic123} on the THuman2.0 dataset~\cite{tao2021function4d}. 
Our results showcase photorealistic images with consistent views that are consistent with the input images.
% We show the full 360-degree view generation results of more subjects in our \emph{supplementary material}.
% \changil{Add citations next to the baseline names above.}
% \changil{I see that we used the results of ELICIT that were provided by the authors in Figure 7, but why did we not use the same identities in Figure 6? It could be a single figure?}\badour{because in that subset are results are not great as in these results.}
% \changil{Do we have more results in the supplementary material? Let's mention it in the caption if we do.}
}
\label{fig:thuman}
\end{figure*}

==> figures/results_unsplash.tex <==
\begin{figure*}[t]
\centering

%%%% INPUT %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{Input}}}  \hfill
\mpage{0.05}{}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=270 0 270 0, clip]{images/unsplash_blur/input/benjamin-rascoe-Z7b2Px6yT40-unsplash.png}}\hfill
\mpage{0.05}{}\hfill
\mpage{0.05}{}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=270 0 270 0, clip]{images/unsplash_blur/input/leah-hetteberg-cZL53ayxS44-unsplash.png}}\hfill
\mpage{0.05}{}\hfill
\mpage{0.05}{}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=270 0 270 0, clip]{images/unsplash_blur/input/leah-hetteberg-Fbl1i1WhAQ8-unsplash.png}}\hfill
\mpage{0.05}{}\hfill
\mpage{0.05}{}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=270 0 270 0, clip]{images/unsplash_blur/input/nassim-boughazi-dodzmVtjoKs-unsplash.png}}\hfill
\mpage{0.05}{}\hfill
\mpage{0.05}{}\hfill
\mpage{0.07}{\includegraphics[width=\linewidth, trim=270 0 270 0, clip]{images/unsplash_blur/input/marcel-strauss-_x9ITyYBcN4-unsplash.png}}\hfill
\mpage{0.05}{}\\
 
%%%% PIFu %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{PIFu~\shortcite{saito2019pifu}}}}  \hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/benjamin-rascoe-Z7b2Px6yT40-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/benjamin-rascoe-Z7b2Px6yT40-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/benjamin-rascoe-Z7b2Px6yT40-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/leah-hetteberg-cZL53ayxS44-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/leah-hetteberg-cZL53ayxS44-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/leah-hetteberg-cZL53ayxS44-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/leah-hetteberg-Fbl1i1WhAQ8-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/leah-hetteberg-Fbl1i1WhAQ8-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/leah-hetteberg-Fbl1i1WhAQ8-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/marcel-strauss-_x9ITyYBcN4-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/marcel-strauss-_x9ITyYBcN4-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/marcel-strauss-_x9ITyYBcN4-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/nassim-boughazi-dodzmVtjoKs-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/nassim-boughazi-dodzmVtjoKs-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/pifu/nassim-boughazi-dodzmVtjoKs-unsplash/080.png}}\\


%%%% iper %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{Impersonator++~\shortcite{liu2021liquid}}}}  \hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/benjamin-rascoe-Z7b2Px6yT40-unsplash/pred_00000010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/benjamin-rascoe-Z7b2Px6yT40-unsplash/pred_00000030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/benjamin-rascoe-Z7b2Px6yT40-unsplash/pred_00000080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/leah-hetteberg-cZL53ayxS44-unsplash/pred_00000010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/leah-hetteberg-cZL53ayxS44-unsplash/pred_00000030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/leah-hetteberg-cZL53ayxS44-unsplash/pred_00000080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/leah-hetteberg-Fbl1i1WhAQ8-unsplash/pred_00000010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/leah-hetteberg-Fbl1i1WhAQ8-unsplash/pred_00000030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/leah-hetteberg-Fbl1i1WhAQ8-unsplash/pred_00000080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/marcel-strauss-_x9ITyYBcN4-unsplash/pred_00000010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/marcel-strauss-_x9ITyYBcN4-unsplash/pred_00000030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/marcel-strauss-_x9ITyYBcN4-unsplash/pred_00000080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/nassim-boughazi-dodzmVtjoKs-unsplash/pred_00000010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/nassim-boughazi-dodzmVtjoKs-unsplash/pred_00000030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/iper/nassim-boughazi-dodzmVtjoKs-unsplash/pred_00000080.png}}\\

%%%% texture %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{TEXTure~\shortcite{richardson2023texture}}}}  \hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/benjamin-rascoe-Z7b2Px6yT40-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/benjamin-rascoe-Z7b2Px6yT40-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/benjamin-rascoe-Z7b2Px6yT40-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/leah-hetteberg-cZL53ayxS44-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/leah-hetteberg-cZL53ayxS44-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/leah-hetteberg-cZL53ayxS44-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/leah-hetteberg-Fbl1i1WhAQ8-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/leah-hetteberg-Fbl1i1WhAQ8-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/leah-hetteberg-Fbl1i1WhAQ8-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/marcel-strauss-_x9ITyYBcN4-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/marcel-strauss-_x9ITyYBcN4-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/marcel-strauss-_x9ITyYBcN4-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/nassim-boughazi-dodzmVtjoKs-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/nassim-boughazi-dodzmVtjoKs-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/texture/nassim-boughazi-dodzmVtjoKs-unsplash/080.png}}\\

%%%% Magic123 %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{Magic123~\shortcite{qian2023magic123}}}}  \hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/benjamin-rascoe-Z7b2Px6yT40-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/benjamin-rascoe-Z7b2Px6yT40-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/benjamin-rascoe-Z7b2Px6yT40-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/leah-hetteberg-cZL53ayxS44-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/leah-hetteberg-cZL53ayxS44-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/leah-hetteberg-cZL53ayxS44-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/leah-hetteberg-Fbl1i1WhAQ8-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/leah-hetteberg-Fbl1i1WhAQ8-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/leah-hetteberg-Fbl1i1WhAQ8-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/marcel-strauss-_x9ITyYBcN4-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/marcel-strauss-_x9ITyYBcN4-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/marcel-strauss-_x9ITyYBcN4-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/nassim-boughazi-dodzmVtjoKs-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/nassim-boughazi-dodzmVtjoKs-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/magic123/nassim-boughazi-dodzmVtjoKs-unsplash/080.png}}\\

\vspace{-1mm}


%%%% S3F %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{S3F~\shortcite{corona2022structured}}}}  \hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/benjamin-rascoe-Z7b2Px6yT40-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/benjamin-rascoe-Z7b2Px6yT40-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/benjamin-rascoe-Z7b2Px6yT40-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/leah-hetteberg-cZL53ayxS44-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/leah-hetteberg-cZL53ayxS44-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/leah-hetteberg-cZL53ayxS44-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/leah-hetteberg-Fbl1i1WhAQ8-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/leah-hetteberg-Fbl1i1WhAQ8-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/leah-hetteberg-Fbl1i1WhAQ8-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/marcel-strauss-_x9ITyYBcN4-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/marcel-strauss-_x9ITyYBcN4-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/marcel-strauss-_x9ITyYBcN4-unsplash/080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/nassim-boughazi-dodzmVtjoKs-unsplash/010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/nassim-boughazi-dodzmVtjoKs-unsplash/030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=380 0 380 0, clip]{images/unsplash_blur/s3f/nassim-boughazi-dodzmVtjoKs-unsplash/080.png}}\\

\vspace{-1mm}

%%%% ours %%%%
\mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{Ours}}}  \hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/benjamin-rascoe-Z7b2Px6yT40-unsplash/view_010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/benjamin-rascoe-Z7b2Px6yT40-unsplash/view_030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/benjamin-rascoe-Z7b2Px6yT40-unsplash/view_080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/leah-hetteberg-cZL53ayxS44-unsplash/view_010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/leah-hetteberg-cZL53ayxS44-unsplash/view_030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/leah-hetteberg-cZL53ayxS44-unsplash/view_080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/leah-hetteberg-Fbl1i1WhAQ8-unsplash/view_010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/leah-hetteberg-Fbl1i1WhAQ8-unsplash/view_030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/leah-hetteberg-Fbl1i1WhAQ8-unsplash/view_080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/marcel-strauss-_x9ITyYBcN4-unsplash/view_010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/marcel-strauss-_x9ITyYBcN4-unsplash/view_030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/marcel-strauss-_x9ITyYBcN4-unsplash/view_080.png}}\hfill
\hspace{2mm}
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/nassim-boughazi-dodzmVtjoKs-unsplash/view_010.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/nassim-boughazi-dodzmVtjoKs-unsplash/view_030.png}}\hfill
\mpage{0.05}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash_blur/ours/nassim-boughazi-dodzmVtjoKs-unsplash/view_080.png}}\\

\vspace{-1mm}

\caption{\textbf{Visual comparison on in-the-wild images from Unsplash.}
We compare our 3D human digitization approach with prior methods~\cite{saito2019pifu,liu2021liquid,richardson2023texture,corona2022structured,qian2023magic123} on images in-the-wild to showcase the generalizability of our approach.
Our approach demonstrates high-resolution photorealistic results that preserve the appearance of the input image. 
%Images from Unsplash.
% We show the full 360-degree view generation results of more subjects in our \emph{supplementary material}.
% \changil{Add citations next to baseline names above.}
% \changil{Do we have more results in the supplementary material? Let's mention it in the caption if we do.}
}
\label{fig:unsplash}
\end{figure*}

==> figures/results_unsplash_rows.tex <==
\begin{figure*}[t]
\centering

% %%%% 
% \mpage{0.1}{\includegraphics[width=\linewidth, trim=270 0 270 0, clip]{images/unsplash/input/mitchell-luo-CMng5BzPv1o-unsplash.png}}\hfill
% \mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/mitchell-luo-CMng5BzPv1o-unsplash/010.png}}\hfill
% \mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/mitchell-luo-CMng5BzPv1o-unsplash/030.png}}\hfill
% \mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/mitchell-luo-CMng5BzPv1o-unsplash/080.png}}\hfill
% \hspace{1mm}
% \mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/asal-mshk-j5YvQDGYNsY-unsplash/pred_00000010.png}}\hfill
% \mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/asal-mshk-j5YvQDGYNsY-unsplash/pred_00000030.png}}\hfill
% \mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/asal-mshk-j5YvQDGYNsY-unsplash/pred_00000080.png}}\hfill
% \hspace{1mm}
% \mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/id_00004235/010.png}}\hfill
% \mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/id_00004235/030.png}}\hfill
% \mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/id_00004235/080.png}}\hfill
% \hspace{1mm}
% \mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/mitchell-luo-CMng5BzPv1o-unsplash/view_010.png}}\hfill
% \mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/mitchell-luo-CMng5BzPv1o-unsplash/view_030.png}}\hfill
% \mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/mitchell-luo-CMng5BzPv1o-unsplash/view_080.png}}\hfill
% \\

%%%% 
\mpage{0.1}{\includegraphics[width=\linewidth, trim=270 0 270 0, clip]{images/unsplash/input/benjamin-rascoe-Z7b2Px6yT40-unsplash.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/benjamin-rascoe-Z7b2Px6yT40-unsplash/010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/benjamin-rascoe-Z7b2Px6yT40-unsplash/030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/benjamin-rascoe-Z7b2Px6yT40-unsplash/080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/benjamin-rascoe-Z7b2Px6yT40-unsplash/pred_00000010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/benjamin-rascoe-Z7b2Px6yT40-unsplash/pred_00000030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/benjamin-rascoe-Z7b2Px6yT40-unsplash/pred_00000080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/benjamin-rascoe-Z7b2Px6yT40-unsplash/010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/benjamin-rascoe-Z7b2Px6yT40-unsplash/030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/benjamin-rascoe-Z7b2Px6yT40-unsplash/080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/benjamin-rascoe-Z7b2Px6yT40-unsplash/view_010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/benjamin-rascoe-Z7b2Px6yT40-unsplash/view_030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/benjamin-rascoe-Z7b2Px6yT40-unsplash/view_080.png}}\hfill
\\

%%%% 
\mpage{0.1}{\includegraphics[width=\linewidth, trim=270 0 270 0, clip]{images/unsplash/input/leah-hetteberg-cZL53ayxS44-unsplash.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/leah-hetteberg-cZL53ayxS44-unsplash/010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/leah-hetteberg-cZL53ayxS44-unsplash/030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/leah-hetteberg-cZL53ayxS44-unsplash/080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/leah-hetteberg-cZL53ayxS44-unsplash/pred_00000010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/leah-hetteberg-cZL53ayxS44-unsplash/pred_00000030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/leah-hetteberg-cZL53ayxS44-unsplash/pred_00000080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/leah-hetteberg-cZL53ayxS44-unsplash/010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/leah-hetteberg-cZL53ayxS44-unsplash/030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/leah-hetteberg-cZL53ayxS44-unsplash/080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/leah-hetteberg-cZL53ayxS44-unsplash/view_010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/leah-hetteberg-cZL53ayxS44-unsplash/view_030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/leah-hetteberg-cZL53ayxS44-unsplash/view_080.png}}\hfill
\\

% %%%% 
\mpage{0.1}{\includegraphics[width=\linewidth, trim=270 0 270 0, clip]{images/unsplash/input/leah-hetteberg-Fbl1i1WhAQ8-unsplash.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/leah-hetteberg-Fbl1i1WhAQ8-unsplash/010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/leah-hetteberg-Fbl1i1WhAQ8-unsplash/030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/leah-hetteberg-Fbl1i1WhAQ8-unsplash/080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/leah-hetteberg-Fbl1i1WhAQ8-unsplash/pred_00000010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/leah-hetteberg-Fbl1i1WhAQ8-unsplash/pred_00000030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/leah-hetteberg-Fbl1i1WhAQ8-unsplash/pred_00000080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/leah-hetteberg-Fbl1i1WhAQ8-unsplash/010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/leah-hetteberg-Fbl1i1WhAQ8-unsplash/030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/leah-hetteberg-Fbl1i1WhAQ8-unsplash/080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/leah-hetteberg-Fbl1i1WhAQ8-unsplash/view_010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/leah-hetteberg-Fbl1i1WhAQ8-unsplash/view_030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/leah-hetteberg-Fbl1i1WhAQ8-unsplash/view_080.png}}\hfill
\\

%%%% 
\mpage{0.1}{\includegraphics[width=\linewidth, trim=270 0 270 0, clip]{images/unsplash/input/nassim-boughazi-dodzmVtjoKs-unsplash.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/nassim-boughazi-dodzmVtjoKs-unsplash/010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/nassim-boughazi-dodzmVtjoKs-unsplash/030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/nassim-boughazi-dodzmVtjoKs-unsplash/080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/nassim-boughazi-dodzmVtjoKs-unsplash/pred_00000010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/nassim-boughazi-dodzmVtjoKs-unsplash/pred_00000030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/nassim-boughazi-dodzmVtjoKs-unsplash/pred_00000080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/nassim-boughazi-dodzmVtjoKs-unsplash/010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/nassim-boughazi-dodzmVtjoKs-unsplash/030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/nassim-boughazi-dodzmVtjoKs-unsplash/080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/nassim-boughazi-dodzmVtjoKs-unsplash/view_010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/nassim-boughazi-dodzmVtjoKs-unsplash/view_030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/nassim-boughazi-dodzmVtjoKs-unsplash/view_080.png}}\hfill
\\

%%%% 
\mpage{0.1}{\includegraphics[width=\linewidth, trim=270 0 270 0, clip]{images/unsplash/input/marcel-strauss-_x9ITyYBcN4-unsplash.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/marcel-strauss-_x9ITyYBcN4-unsplash/010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/marcel-strauss-_x9ITyYBcN4-unsplash/030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/pifu/marcel-strauss-_x9ITyYBcN4-unsplash/080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/marcel-strauss-_x9ITyYBcN4-unsplash/pred_00000010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/marcel-strauss-_x9ITyYBcN4-unsplash/pred_00000030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/iper/marcel-strauss-_x9ITyYBcN4-unsplash/pred_00000080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/marcel-strauss-_x9ITyYBcN4-unsplash/010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/marcel-strauss-_x9ITyYBcN4-unsplash/030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/texture/marcel-strauss-_x9ITyYBcN4-unsplash/080.png}}\hfill
\hspace{1mm}
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/marcel-strauss-_x9ITyYBcN4-unsplash/view_010.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/marcel-strauss-_x9ITyYBcN4-unsplash/view_030.png}}\hfill
\mpage{0.06}{\includegraphics[width=\linewidth, trim=350 0 350 0, clip]{images/unsplash/ours/marcel-strauss-_x9ITyYBcN4-unsplash/view_080.png}}\hfill
\\




\mpage{0.1}{\small{Input}}\hfill
\mpage{0.2}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~PIFu~\shortcite{saito2019pifu}~~}}}$}\hfill
\mpage{0.2}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~Impersonator++~\shortcite{liu2021liquid}~~}}}$}\hfill
\mpage{0.2}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~TEXTure~\shortcite{richardson2023texture}~~}}}$}\hfill
\mpage{0.2}{$\underbrace{\hspace{\textwidth}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~Ours~~}}}$}\\





\caption{\textbf{Visual comparison on in-the-wild images from Unsplash.}
We compare our 3D human digitization approach with prior methods~\cite{saito2019pifu,liu2021liquid,richardson2023texture} on images in-the-wild to showcase the generalizability of our approach.
Our approach demonstrates high-resolution photorealistic results that preserve the appearance of the input image. Images from Unsplash.
We show the full 360-degree view generation results of more subjects in our \emph{supplementary material}.
% \changil{Add citations next to baseline names above.}
% \changil{Do we have more results in the supplementary material? Let's mention it in the caption if we do.}
}
\label{fig:unsplash}
\end{figure*}

==> figures/shapeguidance.tex <==
\begin{figure}[t]
\centering


% \mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{Without reconstruction loss}}}  \hfill
\mpage{0.14}{\includegraphics[width=\linewidth, trim=100 0 100 0, clip]{images/details_id_00002818_blur/masked_inputs_45.png}}\hfill
\mpage{0.14}{\includegraphics[width=\linewidth, trim=100 0 100 0, clip]{images/details_id_00002818_blur/inpaint_merged.png}}\hfill
\mpage{0.14}{\includegraphics[width=\linewidth, trim=100 0 100 0, clip]{images/details_id_00002818_blur/inpaint_normal_merged.png}}\hfill
\mpage{0.14}{\includegraphics[width=\linewidth, trim=100 0 100 0, clip]{images/details_id_00002818_blur/inpaint_edge_merged.png}}\hfill
\mpage{0.14}{\includegraphics[width=\linewidth, trim=100 0 100 0, clip]{images/details_id_00002818_blur/inpaint_normaledge_merged.png}}\\



% \mpage{0.03}{\raisebox{0pt}{\rotatebox{90}{}}}  \hfill
\mpage{0.14}{\footnotesize{Input}}\hfill
\mpage{0.14}{\footnotesize{(a) No guidance}}\hfill
\mpage{0.14}{\footnotesize{(b) Normal}}\hfill
\mpage{0.14}{\footnotesize{(c) Silhouette}}\hfill
\mpage{0.14}{\footnotesize{(d) Normal and silhouette}}\\
\vspace{-2mm}

\captionof{figure}{
\textbf{Shape-guided diffusion inpainting.}
To synthesize the unseen appearance in a new view, we use a pretrained inpainting diffusion model. 
% motivation
With no guidance, the inpainted regions often do not preserve the shape (red silhouette) nor the structural details of the 3D geometry (a). 
% controlnet
% To address this, we use ControlNet~\shortcite{zhang2023adding} to incorporate additional control signals into the diffusion model.
% add normal maps
If we use normal maps as a control signal for ControlNet~\shortcite{zhang2023adding} (b), the inpainted region preserves the structural details of the mesh (e.g., fingers), but not the shape of the human body.
% \changil{What are the ``structural details''? It's hard to see the difference between (a) and (b). Can we add markers to point readers to them?}
% \badour{structural details are for example where the hands are or whether you are looking at the front (structural details of face=nose, lips, hair, etc.) or back (more smoother structure). These are available with the normal map but not the edge countor. The normal will therefore preserve thise "structure" but the edge sil will just specify the shape.}
% \changil{I think we should this in the caption (in a short, summarized form). Can we add a marker in the figure to show what to look for? Or better, do we have an example with a more obvious difference?}
% add edges of the mesh silhouette
Using the silhouette map preserves the shape of the human body, but not the structural details of the mesh (c).
% what we did
We propose to use both normal and silhouette maps to guide the inpainting model to respect the underlying 3D geometry (d).
}
\label{fig:shapeguidance}
\end{figure}

==> setup/graphicspath.tex <==
\graphicspath{{figures}, {examples}}


==> setup/package.tex <==
% Fix "undefined control sequence \Everyshipout".
% \usepackage{everyshi}

% Figures
% \usepackage{graphicx}
\usepackage{subcaption}
\usepackage{float}
\usepackage[justification=raggedright]{caption}	% makes captions ragged right - thanks to Bryce Lobdell
\usepackage{lscape}                                         % Useful for wide tables or figures.
\usepackage{wrapfig}

% Algorithm
\usepackage[lined,ruled,linesnumbered]{algorithm2e}
\usepackage{animate} %% convert frames to video

% Table and list
\usepackage{booktabs}                   % Publication quality tables
\usepackage{multirow}

\usepackage{makecell}

\usepackage{paralist}
\usepackage{enumitem}
\setlist[enumerate]{itemsep=0mm}

% Math
\usepackage{bm}                          % Make bold, italic math symbols
\usepackage{epsfig}                      % for figures
\usepackage{graphicx}                  % another package that works for figures
\usepackage{times}
\usepackage{mathptmx}
\usepackage{mathtools}
\usepackage{amssymb,amsmath}   % Short math guide for LaTeX ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf

% Fonts
\usepackage{units}
\usepackage{color}
\usepackage{xcolor}

% Comments
\usepackage{comment}

% Hyperlinks
\usepackage{url}  % Hyphenation of URLs.
%\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,pagebackref=true,colorlinks,bookmarks=false]{hyperref}
% \usepackage[pagebackref,breaklinks,colorlinks,linkcolor=blue,citecolor=blue,urlcolor=blue,bookmarks=false]{hyperref}
% \usepackage{authblk}
% \usepackage{slashbox}
% \usepackage{xspace}
% \usepackage[table]{xcolor}
% \usepackage{setspace}
% \usepackage{grfext}
% \PrependGraphicsExtensions*{.jpg,.png,.PNG}

\usepackage{gensymb}
% \usepackage{emoji}

% \usepackage{times,color}
% \usepackage{parskip}
% %\usepackage{epsfig}
% %\usepackage{psfig}
% %\usepackage[pdftex]{graphicx} % new acmsiggraph.cls
% \usepackage{ifthen}
% %\usepackage[draft]{hyperref} % new acmsiggraph.cls
% \usepackage{float}
% \usepackage{alltt}
% \usepackage{mathenv}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{amsthm}
% %\usepackage{rotating}
% \usepackage{newlfont} % for Box
% %\usepackage{ulem}
% \usepackage{floatflt}
% \usepackage{wrapfig}
% \usepackage{fixltx2e}
% \usepackage{subfig} % for subfloat
% \usepackage{multirow}
% \usepackage{cleveref}
% \usepackage{algorithmic}
% \usepackage{CJKutf8} % Chinese


==> setup/symbols.tex <==
% Define math symbols that appear in the texts

\def\xi{\mathbf{x}_i}
\def\yi{\mathbf{y}_i}

